The final spin from the coalescence of aligned-spin black-hole binaries

Determining the final spin of a black-hole (BH) binary is a question of key importance in astrophysics. Modelling this quantity in general is made difficult by the fact that it depends on the 7-dimensional space of parameters characterizing the two initial black holes. However, in special cases, when symmetries can be exploited, the description can become simpler. For black-hole binaries with unequal masses but with equal spins which are aligned with the orbital angular momentum, we show that the use of recent simulations and basic but exact constraints derived from the extreme mass-ratio limit allow to model this quantity with a simple analytic expression. Despite the simple dependence, the expression models very accurately all of the available estimates, with errors of a couple of percent at most. We also discuss how to use the fit to predict when a Schwarzschild BH is produced by the merger of two spinning BHs, when the total angular momentum of the spacetime ``flips'' sign, or under what conditions the final BH is ``spun-up'' by the merger. Finally, suggest an extension of the fit to include unequal-spin binaries, thus potentially providing a complete description of the final spin from the coalescence of generic black-hole binaries with spins aligned to the orbital angular momentum.

==> Makefile <==
# Makefile for this paper

#
# Note this Makefile always re-TeXs things, even if the .tex files
# haven't changed (and similarly for dvips); this ensures that changes
# to macros, included stuff from other directories, etc, get "used".
# To implement this, we declare the .dvi and .ps files as "PHONY".
#

###############################################################################

.PHONY	: default
default	: ps pdf

.PHONY	: dvi
dvi	:
	latex unequalmass_diagram
#	bibtex unequalmass_diagram
	latex unequalmass_diagram

.PHONY	: ps
ps	: dvi
	dvips -f <unequalmass_diagram.dvi >unequalmass_diagram.ps

.PHONY	: pdf
pdf	: ps
	ps2pdf unequalmass_diagram.ps

########################################

.PHONY	: bib
bib	:
	@test -f bibtex/references.bib \
         || (echo '*** you must have a copy of the AEI numrel "references.bib" file' ; \
             echo '*** accessible under the name "bibtex/references.bib"; you can get this via' ; \
             echo '***    cvs -d:pserver:USERNAME@cvs.aei.mpg.de:numrelcvs checkout bibtex'; \
             echo '*** or by symlinking a checkout from somewhere else'; \
             exit 1)
	@test -f bibtex/apsrev-nourl.bst \
         || (echo '*** you must have a copy of the AEI numrel "bibtex/apsrev-nourl.bst" file' ; \
             echo '*** accessible under the name "bibtex/bibtex/apsrev-nourl.bst"; you can get this via' ; \
             echo '***    cvs -d:pserver:USERNAME@cvs.aei.mpg.de:numrelcvs checkout bibtex'; \
             echo '*** or by symlinking a checkout from somewhere else'; \
             exit 1)
	bibtex unequalmass_diagram

########################################

.PHONY	: clean
clean	:
	-rm unequalmass_diagram.dvi unequalmass_diagram.aux unequalmass_diagram.log unequalmass_diagram.bbl unequalmass_diagram.blg unequalmass_diagram.end unequalmass_diagram.ps unequalmass_diagram.pdf

########################################

.PHONY	: tarball
tarball	:
	tar -cvf - ./unequalmass_diagram.tex \
                   ./unequalmass_diagram.bbl \
                   ./plots/calibration.eps \
                   ./plots/vkick_vs_time.eps \
                   ./plots/vkick_vs_spinratio.eps \
            | gzip >unequalmass_diagram.tar.gz

########################################

